Neural Network Equalizers and Successive Interference Cancellation for Bandlimited Channels with a Nonlinearity

Neural networks (NNs) inspired by the forward-backward algorithm (FBA) are used as equalizers for bandlimited channels with a memoryless nonlinearity. The NN-equalizers are combined with successive interference cancellation (SIC) to approach the information rates of joint detection and decoding (JDD) with considerably less complexity than JDD and other existing equalizers. Simulations for short-haul optical fiber links with square-law detection illustrate the gains.

==> plots/plot_settings.tex <==
\pgfkeys{/pgf/number format/.cd,fixed,precision=1}

\definecolor{mycolor1}{HTML}{0072bd}%
\definecolor{mycolor6}{HTML}{FF0000}%
\definecolor{mycolor5}{HTML}{27ae60}%
\definecolor{mycolorrnn}{HTML}{F5B400}%

\pgfmathsetmacro{\gridwidth}{2.35in}
\pgfmathsetmacro{\gridheight}{1.08in}
\pgfmathsetmacro{\lwidth}{0.45pt}


\pgfplotsset{
   PAM/.style={
    mycolor1,
    line width=\lwidth,
   },
   ASK/.style={
    mycolor6,
    line width=\lwidth,
    },
    QAM/.style={
       mycolor5,
    line width=\lwidth,
    },
    GS/.style={
       densely dashdotted,
       line width=1pt,
    },
    RNN/.style={
        mycolor5,
        mark=*,mark size={1.0pt},mark options={solid,fill=white},line width=0.5pt
    },
    FBA/.style={
        mark=none,mark size={1.1pt},line width=0.5pt, densely dashdotted
    },
    UB/.style={
       line width=\lwidth,
       mark=none,
       black,
       solid
    }
}

\tikzset{
    arr/.style={thick,{Stealth[length=1.2mm, width=1.2mm]}-{Stealth[length=1.2mm, width=1.2mm]}},
    arrR/.style={thick,-{Stealth[length=1.2mm, width=1.2mm]}},
    opacitylabel/.style={
       fill=white, fill opacity=0.8,text opacity=1, draw opacity=1, inner sep=0.5pt
    }}
  
